Immersion Metrics for Virtual Reality

Technological advances in recent years have promoted the development of virtual reality systems that have a wide variety of hardware and software characteristics, providing varying degrees of immersion. Immersion is an objective property of the virtual reality system that depends on both its hardware and software characteristics. Virtual reality systems are currently attempting to improve immersion as much as possible. However, there is no metric to measure the level of immersion of a virtual reality system based on its characteristics. To date, the influence of these hardware and software variables on immersion has only been considered individually or in small groups. The way these system variables simultaneously affect immersion has not been analyzed either. In this paper, we propose immersion metrics for virtual reality systems based on their hardware and software variables, as well as the development process that led to their formulation. From the conducted experiment and the obtained data, we followed a methodology to find immersion models based on the variables of the system. The immersion metrics presented in this work offer a useful tool in the area of virtual reality and immersive technologies, not only to measure the immersion of any virtual reality system but also to analyze the relationship and importance of the variables of these systems.

==> TODOs.tex <==
Paper:
- Citar dataset (listo)
- Subir a arxiv
- ver si se deben llamar Ecuaciones, funciones o fórmulas
se llaman funciones ya fue, porque es TI(x1,...,xn)= (listo)

Supplementary Material:
- Imagenes de las variables (listo)
- Excel de todas las referencias y variables (listo)
